NDSEARCH: Accelerating Graph-Traversal-Based Approximate Nearest Neighbor Search through Near Data Processing

Approximate nearest neighbor search (ANNS) is a key retrieval technique for vector database and many data center applications, such as person re-identification and recommendation systems. It is also fundamental to retrieval augmented generation (RAG) for large language models (LLM) now. Among all the ANNS algorithms, graph-traversal-based ANNS achieves the highest recall rate. However, as the size of dataset increases, the graph may require hundreds of gigabytes of memory, exceeding the main memory capacity of a single workstation node. Although we can do partitioning and use solid-state drive (SSD) as the backing storage, the limited SSD I/O bandwidth severely degrades the performance of the system. To address this challenge, we present NDSEARCH, a hardware-software co-designed near-data processing (NDP) solution for ANNS processing. NDSEARCH consists of a novel in-storage computing architecture, namely, SEARSSD, that supports the ANNS kernels and leverages logic unit (LUN)-level parallelism inside the NAND flash chips. NDSEARCH also includes a processing model that is customized for NDP and cooperates with SEARSSD. The processing model enables us to apply a two-level scheduling to improve the data locality and exploit the internal bandwidth in NDSEARCH, and a speculative searching mechanism to further accelerate the ANNS workload. Our results show that NDSEARCH improves the throughput by up to 31.7x, 14.6x, 7.4x 2.9x over CPU, GPU, a state-of-the-art SmartSSD-only design, and DeepStore, respectively. NDSEARCH also achieves two orders-of-magnitude higher energy efficiency than CPU and GPU.

==> 3.OverallArch_ProcessingModel.tex <==
\section{System Overview}
\label{sec:overall}
\input{fig/OverallLUNNCSR}
In this section, we introduce \design for accelerating graph-traversal-based ANNS. 
%First, we present the overall architecture of \design based on SmartSSD~\cite{}. 
%\yt{LUNCSR}
%Then, we propose a new processing model for graph traversal based ANNS, considering both the architecture of \design and the generality of ANNS algorithms.
%\subsection{Overall architecture}
Our \design is based on the architecture of SmartSSD~\cite{lee2020smartssd}, as illustrated in Fig.~\ref{fig:overallnluncsr}(a).
SmartSSD consists of an FPGA device and an SSD device.
The FPGA and the SSD is connected via a private PCIe 3.0$\times$4 link. 
As aforementioned, we extract three kernels from the workload of graph-traversal-based ANNS, graph traversal, distance computation, and bitonic sort. 
We modify the original SSD as \ssd and offload the graph traversal and distance computation kernels to it.
The graph traversal kernel is executed in the embedded cores with additional customized logic (Vgenerator and Allocator in Section~\ref{sec:micro}) in the SSD.
The distance computation kernel runs on the Search-in-Nand (SiN) engines where LUN-level accelerators are developed. Each SSD channel consists of four SiN engines. \ssd outputs the result lists of each query to the FPGA. The result list of one query only needs to contain the index of the query, the indices of the query's candidate neighbors and the scalar distances between the query and the candidates. The feature vectors of query and targeted vertices are ``filtered" by the \ssd so the limited PCIe bandwidth is acceptable for transmitting the scalar distances, which could be as low as $1/32$ of the data transferred via PCIe link in~\cite{smartSSDKNN}.
The FPGA executes the bitonic sorting kernel and returns the top-k neighbors of each query to the host.
%and then allocates the queries to different LUNs.
%The IDs are sent to corresponding LUNs to access the feature vectors in the flash chip.
%Then, the distance computation kernel is executed at LUN level accelerator to compute the distance between the queries and the fetched vertices in the LUNs.
%The computed distance is sent back from each LUN to the embedded CPU to find the nearest vertex for this iteration.
%The result list is kept in the main memory of the embedded CPU and sent to the FPGA.
%The FPGA process these information with the \textit{bitonic sort} kernel.
%In this case, all the feature vector are accessed and processed locally within the SSD device and only the calculated distance information need to be transferred.
%FPGA device to execute the bitonic sorting kernel.
%As a high parallel sorting algorithm, bitonic sorting kernel sorts the distances in the candidate lists of each queries utilizing the high parallelism and flexibility of FPGA.
%After receiving a batch of queries sent from the host, \ssd works like a "filter" that only outputs a batch of lists instead of all the vertices in each searching trace to the FPGA via the P2P link. 
%The bitonic sorting kernel on FPGA is similar to ~\cite{}, which is not the focus of this work.





==> 7.RelatedWork.tex <==
\section{Other Related Work}
\label{sec:related}
There are many other works related to the acceleration of ANNS. Facebook proposes a framework - Faiss~\cite{johnson2019billion} which was initially designed for supporting various ANNS algorithms on GPU. Due to the limited memory capacity of VRAM on GPU, Faiss usually adopts the approach of compressing the data like product quantization (PQ). HM-ANN~\cite{ren2020hm}  is proposed to utilize the memory hierarchy and the combination of heterogeneous memory to accelerate ANNS. It uses a persistent memory module (PMM), which has higher bandwidth and lower read latency than SSD, to store the vertices without any data compression and uses DRAM as a hardware-managed cache to PMM. Recently, a specialized architecture, ANNA~\cite{ANNA}, is proposed with a delicately designed dataflow pipeline and efficient data reuse to further accelerate Faiss. 

%\noindent \textbf{NDP accelerators.}
%NDP accelerators usually refer to the accelerators built near/in the storage. MithriLog~\cite{kang2021near} adopts the architecture of SmartSSD~\cite{lee2020smartssd}, adding an FPGA board near the SSD, to accelerate log analytics. Although our work also utilizes SmartSSD, we focus more on the architecture design in SSD to exploit the high internal bandwidth of SSD. Parabit~\cite{gao2021parabit} modifies the read circuits of flash chips in SSD to develop bit operations like AND, XOR and etc. However, the bit operation is too simple to support relatively complex computations like MAC. There are some NDP accelerators that are developed from the software side. For example, RecSSD~\cite{wilkening2021recssd} develops the accelerator in the FTL layer on the embedded cores of SSD without any extra hardware implementation.
\label{related}

==> fig/DiffConfig.tex <==
\begin{figure}[t]
	\begin{center}	
		\includegraphics[width=0.9\columnwidth]{fig/DiffConfig_.pdf}
		\hspace{0em}
		\vspace{0em}
		\caption{Speedup normalized to \design with page size set to 2KB. The memory organizations of each configuration are adjusted accordingly to ensure the same memory capacity.}
		\label{DiffConfig}
	\end{center}	
	\vspace{-1em}
\end{figure} 

==> fig/Overall.tex <==
\begin{figure}[t]
	\begin{center}	
		\includegraphics[width=\columnwidth]{fig/Overall.pdf}
		\vspace{-1em}
		\caption{Overall arch...}
		\label{Overall}
	\end{center}	
	\vspace{-2.5em}
\end{figure} 
